Competitive DER Aggregation for Participation in Wholesale Markets

The problem of the large-scale aggregation of the behind-the-meter demand and generation resources by a distributed-energy-resource aggregator (DERA) is considered. As a profit-seeking wholesale market participant, a DERA maximizes its profit while providing competitive services to its customers with higher consumer/prosumer surpluses than those offered by the distribution utilities or community choice aggregators. A constrained profit maximization program for aggregating behind-the-meter generation and consumption resources is formulated, from which payment functions for the behind-the-meter consumptions and generations are derived. Also obtained are DERA's bid and offer curves for its participation in the wholesale energy market and the optimal schedule of behind-the-meter resources. It is shown that the proposed DERA's aggregation model can achieve market efficiency equivalent to that when its customers participate individually directly in the wholesale market.

==> Bidding_v0.tex <==
\subsection{DERA bids in the wholesale market}

\subsubsection{Price taker DERA}

A price taker DERA can choose to provide quantity bids to the wholesale market with optimal generation $P=-\sum_{i=1}^N P_i^{p*}$. Additionally, from (\ref{WholesaleBid}), DERA can also compute the supply function with

$
P=\left\{\begin{matrix}
R -\sum_{i=1}^N (\frac{\alpha-\pi}{\beta}), & if~\pi\le \alpha\\
R, & if~\pi> \alpha
\end{matrix}\right.,
$

$
C'(P)=\left\{\begin{matrix}\frac{\beta}{N}P+\alpha-\frac{\beta R}{N}, & if~P\le R\\
+\infty, & if~P> R
\end{matrix}\right.,\\
$
% $
% C(P)=\frac{\beta}{2N}P^2+(\alpha-\frac{\beta R}{N})P,\\
% $
% $
% C(P)=\left\{\begin{matrix}
% \alpha P + N\alpha ln(P+R-N), &if~ P>N-R \\ 
% % not define, &if~ P=N-R \\ 
% \alpha P - N\alpha ln(N-R-P), &if~ P<N-R 
% \end{matrix}\right.
% $
where $R=\sum_i P^r_i$. And the optimal DERA bidding curve $C'(P)$ when $N=1000$ was shown in Fig.\ref{fig:DERAbiddingCurve}. At competitive equilibrium for the wholesale market, DERA revealed those bidding curves to ISO. The slope was decided by parameters of the prosumer utility function $\beta$ and the number of aggregated prosumers $N$. The intersection of the bidding curve with the y-axis was $(0, \alpha-\frac{\beta R}{N})$.
% \scriptsize{
\begin{figure*}[thb] 
\centering
% \begin{psfrags}
% \scalefig{0.45}\epsfbox{Figs/DERABids3.eps}
% \end{psfrags}
\scalebox{0.43}{\includegraphics{Figs/WholesaleBid.eps}}
 \vspace{-1.5em}
\caption{\scriptsize Optimal Bidding curve for price taker DERA when $N=1000$.}
\label{fig:DERAbiddingCurve}
\end{figure*}
% }
When $\gamma=0$ or $P^r_i=0$, the DERA was a consumer with the same optimal bidding curves.And in all other parameter setting for $\gamma$ ,and $P^r_i$, this DERA can generate to the maximum of $R$ kWh. When $\alpha-\frac{\beta R}{N}<0$, the intersection of the DERA bidding curve with the y-axis is negative. This means DERA tended to generate with even a negative price, reflecting redundant renewable energy to be injected to the power network. When $\alpha-\frac{\beta R}{N}>0$, the intersection of the DERA bidding curve with the y-axis is positive. This means DERA tended to withdraw energy from the power network because of the lack of DER generation internally.


\subsubsection{Price maker DERA}

\textcolor{red}{revised to consider some DERA is producer and some is consumer, satisfy assumption \ref{lemma:SFE_C2}}
In the previous section, DERA had a linear supply function. And here we established a toy example to compute the supply function equilibrium for price maker DERA by assuming three are three wholesale market participants ignoring capacity limits. And then we compared cases for price maker strategic bidding results at SFE, and non-stategic truthful bidding result mimicking CE.

Consider two DERAs indexed by $n=1,2$ in the wholesale market with $P^r_i-\frac{\alpha_i}{\beta_i}=0, \forall i$ for the aggregated homogeneous prosumers. It had supply function $P_n=w_n\pi$ and truthful cost $C(P_n)=\frac{1}{2w_n}P_n^2, n=1,2$ where $w_n=N/\beta_i$. And assume there's another wholesale market participant indexed by $n=3$ with $C_3(P_3)=\frac{1}{2w_3}P_3^2$.

We can solve for the SFE, where the bid-in curve from those three market participants are $\tilde{C}_k(x_k)=\frac{1}{2\tilde{w}_k}x_k^2, \forall k=1,2,3$.  Let $w_3=0.05w_1$, inelastic demand $D=2.5MW$ and the number of aggregated prosumers for eacch DERA be $N=10000$. Fig.\ref{fig:SFE} shows optimal bidding results for DERA at CE and SFE. Solve the optimization (\ref{eq:SFE_thmC}), we had market clearing quantity, price, and optimal DERA bids at SFE. 
% And the optimal bid-in parameters were $\tilde{w}_3=\frac{818}{1503},\tilde{w}_1=\tilde{w}_2=\frac{463}{368}.$ 
%As for the CE where individuals bid truthfully, we had $\bar{x}_3=\frac{3}{4}kWh,\bar{x}_2=\bar{x}_1=\frac{1}{8}kWh, \bar{\pi}=0.03 \$/kWh.$ 
%  $x_1^*= \frac{656}{3689},x_2^*=x_3^*= \frac{571}{1389}$. $\pi^*=0.3267\$/kWh.$ 
% And the optimal bid-in parameters are $\tilde{b}_3=\frac{6+ 8r - 2\sqrt{16 r + 9}}{c r (5+ 8r -\sqrt{16 r + 9})}=\frac{818}{1503},\tilde{b}_1=\tilde{b}_2=-\frac{3 + 4 r - \sqrt{16 r + 9}}{c r (1- \sqrt{16 r + 9})}=\frac{463}{368}.$ And for DERA, the dispatch at SFE is $x_1^*=\frac{571}{1389}kWh$. 
% We have $x^*_3=\frac{-1+\sqrt{16r+9}}{8r+4}D=\frac{656}{3689}kWh,x^*_2=x^*_1=\frac{8r+5-\sqrt{16r+9}}{16r+8}D=\frac{571}{1389}kWh$, and the wholesale market price is $\pi^*=\frac{D-q_1^*}{D-2q_1^*}rcq_1^*=512/1567=0.3267\$/kWh.$ 
% So profit of DERA from the wholesale market is $\pi^*x^*_1-\frac{1}{2}c(x^*_1)^2+C=\frac{251}{2201}+C\$$
% As for the competitive equilibrium we have $\bar{x}_3=\frac{rD}{r+2},\bar{x}_2=\bar{x}_1=\frac{D}{r+2}, \bar{\pi}=c\bar{x}=\frac{rcD}{r+2}.$ 
% And profit of DERA from the wholesale market is $\pi^*x^*_1-\frac{1}{2}c(x^*_1)^2+C=\frac{3}{1600}+C\$$.\textcolor{red}{check if the dispatch and price are the same with the price taker model equations} 
Because we only had 3 wholesale market participants and each of them had huge market power. So the profit of DERA under CE with price taker assumption was much less than that under SFE with price maker assumption. The market clearing price also increased dramatically at SFE compared to CE. Besides, from (\ref{eq:DERAFixRateGP}), we know the aggregated prosumers had the same surplus under the price taker and price maker assumption. 
% \scriptsize{
\begin{figure}[thb] 
\centering
% \begin{psfrags}
% \scalefig{0.45}\epsfbox{Figs/DERABids3.eps}
% \end{psfrags}
\scalebox{0.36}{\includegraphics{Figs/SFE_CE2.eps}}
%  \vspace{-1.5em}
\caption{\scriptsize Optimal bidding results for DERA in CE and SFE.}
\label{fig:SFE}
\end{figure}
% }
% In the DERA aggregation, the aggregation cost of DERA is $ \omega^{0}_i(P^{H}_i)=U_i(P^r_i-P^{H}_i)-S_i^{P}(P^r_i)-\epsilon$. So at the SFE, we have $ \omega^{0}_i(x^*_i)=U_i(P^r_i-x^*_i)-S_i^{P}(P^r_i)-\epsilon$. This is also the energy bill to households, which will be $U(1-\frac{1}{8})-U(1-\frac{571}{1389})= 0.24(\frac{7}{8}-\frac{818}{1389})-0.12(\frac{7}{8}^2-\frac{818}{1389}^2)=\frac{143}{7770}\$$ smaller when DERA is a price maker. Correspondingly household utility is less when DERA is a price maker. 

% Household will directly submit strategic bidding parameter $\tilde{b}_1,\tilde{b}_2$ to the DERA rather than the truthful parameters. And $\omega^{0}_i$ and $\tilde{b}_i$ are all computed distributively at the household-end to preserve the privacy of the household. DERA will submit the aggregated bid-in parameter $\sum_i \tilde{b}_i$ to the wholesale market and collect payment $\omega^{0}_i$ from each household.




% %on case
% We can solve for the SFE, where the bid-in curve from those three market participants are $\tilde{C}_k(x_k)=\frac{1}{2\tilde{w}_k}x_k^2, \forall k=1,2,3$.  Let $w_3=6w_1$, inelastic demand $D=10MWh$ and the number of aggregated prosumers for eacch DERA be $N=10000$. Fig.\ref{fig:SFE} shows optimal bidding results for DERA at CE and SFE. Solve the optimization (\ref{eq:SFE_thmC}), we had market clearing quantity, price, and optimal DERA bids at SFE. 
% % And the optimal bid-in parameters were $\tilde{w}_3=\frac{818}{1503},\tilde{w}_1=\tilde{w}_2=\frac{463}{368}.$ 
% %As for the CE where individuals bid truthfully, we had $\bar{x}_3=\frac{3}{4}kWh,\bar{x}_2=\bar{x}_1=\frac{1}{8}kWh, \bar{\pi}=0.03 \$/kWh.$ 
% %  $x_1^*= \frac{656}{3689},x_2^*=x_3^*= \frac{571}{1389}$. $\pi^*=0.3267\$/kWh.$ 
% % And the optimal bid-in parameters are $\tilde{b}_3=\frac{6+ 8r - 2\sqrt{16 r + 9}}{c r (5+ 8r -\sqrt{16 r + 9})}=\frac{818}{1503},\tilde{b}_1=\tilde{b}_2=-\frac{3 + 4 r - \sqrt{16 r + 9}}{c r (1- \sqrt{16 r + 9})}=\frac{463}{368}.$ And for DERA, the dispatch at SFE is $x_1^*=\frac{571}{1389}kWh$. 
% % We have $x^*_3=\frac{-1+\sqrt{16r+9}}{8r+4}D=\frac{656}{3689}kWh,x^*_2=x^*_1=\frac{8r+5-\sqrt{16r+9}}{16r+8}D=\frac{571}{1389}kWh$, and the wholesale market price is $\pi^*=\frac{D-q_1^*}{D-2q_1^*}rcq_1^*=512/1567=0.3267\$/kWh.$ 
% % So profit of DERA from the wholesale market is $\pi^*x^*_1-\frac{1}{2}c(x^*_1)^2+C=\frac{251}{2201}+C\$$
% % As for the competitive equilibrium we have $\bar{x}_3=\frac{rD}{r+2},\bar{x}_2=\bar{x}_1=\frac{D}{r+2}, \bar{\pi}=c\bar{x}=\frac{rcD}{r+2}.$ 
% % And profit of DERA from the wholesale market is $\pi^*x^*_1-\frac{1}{2}c(x^*_1)^2+C=\frac{3}{1600}+C\$$.\textcolor{red}{check if the dispatch and price are the same with the price taker model equations} 
% Because we only had 3 wholesale market participants and each of them had huge market power. So the profit of DERA under CE with price taker assumption was much less than that under SFE with price maker assumption. The market clearing price also increased dramatically at SFE compared to CE. Besides, from (\ref{eq:DERAFixRateGP}), we know the aggregated prosumers had the same surplus under the price taker and price maker assumption. 
% % \scriptsize{
% \begin{figure}[thb] 
% \centering
% % \begin{psfrags}
% % \scalefig{0.45}\epsfbox{Figs/DERABids3.eps}
% % \end{psfrags}
% \scalebox{0.2}{\includegraphics{Figs/SFE_CE.eps}}
% %  \vspace{-1.5em}
% \caption{\scriptsize Optimal bidding results for DERA in CE and SFE.}
% \label{fig:SFE}
% \end{figure}

==> CCA_v0.tex <==
\subsection{Community choice aggregation}
A community choice aggregation model (CCA) for profit neutral DERA is proposed in \cite{chakraborty2018analysis}. As is explained in (\ref{passiveSurplus}) that $P^{0}_i=d^+_i-P^r_i$ is the net consumption pattern of passive producers. A passive prosumer participating in a CCA has surplus 
\beq\label{CCAsurplus}
S_i^{pc}=\left\{\begin{matrix}
U_i(d^+_i)-\pi^-P^{0}_i-T,&if~\sum_i P^p_i\le 0 \\ 
 U_i(d^+_i)-\pi^+P^{0}_i-T,&if~\sum_i P^p_i> 0 
\end{matrix}\right.
\eeq
If all $M$ prosumers participate CCA and  ${\cal C}-MT=0$, the surplus of utility is $S^u=M((\pi^--\pi)(d_j^+-P^r_j)(1-\gamma)+(\pi^--\pi)(d_i^+-P^r_i)\gamma)$.
% $P^{CCA}(P^r_i)=\left\{\begin{matrix}\pi^+(d_i-P^r_i),& if \sum_i(d_i-P^r_i)>0\\
% \pi^-(d_i-P^r_i),& if \sum_i(d_i-P^r_i)<0
% \end{matrix}\right.$.

% $S_i^{P}(P^r_i)=\left\{\begin{matrix}
% U_i(d^+_i) +\pi^+(P^r_i-d^+_i)-T,&if~ \sum_i(d_i-P^r_i)>0\\ 
%  U_i(d^+_i)+\pi^-(P^r_i-d^+_i)-T,&if~\sum_i(d_i-P^r_i)<0
% \end{matrix}\right.$ 

==> WholesaleModelMaker_v4.tex <==
\subsection{Price maker DERA}

Under a price maker DERA regime, we tackle establishing an optimal DERA bidding curve at supply function equilibrium (SFE) with certain category of  supply function.  We extend the result for SFE with supply function $s(\pi)=w\pi$ \cite{li2015demand} and  $s(\pi)=R-\frac{w}{\pi}$ \cite{johari2011parameterized, johari2004efficiency,  xu2015demand} into a general category $s(\pi)=R-\frac{w}{B(\pi)}$ with capacity limits considered, and this is compatible to DERA aggregating prosumers with various utiltiy functions including quadratic, log and isoelastic utility.

Let $m$ be the index of DERA among the wholesale market participants and $M$ be the total number of wholesale market participants. From (\ref{Q-P}), we get the net production $P_m=s(\pi)$ of DERA under a given wholesale market price $\pi$. \footnote{In this section, superscript $w$ for wholesale market price $\pi$ is dropped for simplicity, and we assume $\pi\geq 0$.} 

\subsubsection{Supply function formulation}
 
Let $[\underline{P}_m,\bar{P}_m]$ be the capacity limit of wholesale participant $m$ with $-\infty<\underline{P}_m\le \bar{P}_m< +\infty$. For DERA we have $\underline{P}_m=R_m-\bar{D}_m$, and $ \bar{P}_m=R_m-\underline{D}_m$. 
\begin{assumption} \label{assume:SFE_C1}
 Assume participates in  wholesale electricity market have supply function $s_m(\pi,w_m)$ parameterized by $w_m$ with:

\begin{itemize}
    \item  $s_m(\pi,w_m)=R_m-\frac{w_m}{B(\pi)}$, where $w_m\geq 0$, $B(\cdot)$ is strictly increasing, differentiable, and invertible. 
    \item $xE'(x)={\cal M}E(x)$, where $E(\cdot):=B^{-1}(\cdot)$ and ${\cal M}$ is a nonzero constant.
    \end{itemize}
\end{assumption}
% So, when $P_m\geq 0$ DERA is injecting energy to the wholesale market with price $\pi$, and when $P_n\le 0$, DERA is withdrawing energy.
Note that when $\wbf=\mathbf{0}$, we have $\pi=0$ and $s_m(0,0)=\frac{R_mD}{\mathbf{1}^\intercal R}$. From (\ref{Q-P})(\ref{WholesaleBid}), the truthful marginal cost of DERA with the proposed DERA model is strongly connected to the utility function $U(\cdot)$ of the aggregated prosumers. Suppose homogeneous aggregated prosumers have log utility functions, DERA from (\ref{Q-P}) gets $s_m(\pi,w_m)=R_m-\frac{w_m}{\pi}$, where $B(\pi)=\pi$, and ${\cal M}=1$. For quadratic utility functions of the aggregated prosumers, DERA has the affine supply function $s_m(\pi,w_m)=R_m+w_m\pi$, where $B(\pi)=-\frac{1}{\pi}$, and ${\cal M}=-1$. For isoelastic utility functions of the aggregated prosumers, DERA has the supply function $s_m(\pi,w_m)=R_m-w_m \pi^{\frac{-1}{\eta}}, \eta\geq 0, \eta\neq1$, where $B(\pi)=\pi^{\frac{1}{\eta}}$, and ${\cal M}=1$.

% $U_i(P^d_i)=log(P^d_i)$
% $U_i(P^d_i)=\alpha_i-\frac{1}{2}\beta_i P^d_i^2$
% $ U(P^d_i)=\frac{w_n^{1-\alpha}P^d_i^\alpha-\alpha}{\alpha}$


\subsubsection{Supply function equilibrium}

The profit of wholesale market participant $m$ is
\beq
Q_m(w_m;\wbf_{-m})=\pi(\wbf)s_m(\wbf)-C_m(s_n(\wbf)),\eeq
where $\wbf_{-m}:=(w_1,...,w_{m-1},w_{m+1},...,w_M)$ and $C_m(\cdot)$ is the truthful cost function. SFE is one kind of Nash equilibrium with the following definition:
\begin{definition}
A vector $\wbf^*$ is a (pure-strategy) Nash equilibrium if $Q_m(w^*_m,\wbf^*_{-m})= \max_{\underlined w_m\geq 0} Q_m(w_m,\wbf^*_{-m}), \forall m\in \{1,...,M\}$.
\end{definition}
 To guarantee the existence of SFE and reduce the computation burden for SFE, we have the following assumptions:
\begin{assumption} \label{assump:SFE_C2}
Assume coefficients of wholesale market participants have that
\begin{itemize}
    \item $\sum_{j=1}^M w_j\neq 0$.
    \item $\sum_{j\neq m} R_j\geq {\cal D} $, if $B(\cdot)$ is unbounded above.    
    \item The truthful cost function $C_m:(-\infty, \infty)\rightarrow (-\infty, \infty), \forall m$ is continuous and convex with $C_m(0)=0$. Also $C_m(\cdot)$ is strictly increasing over the positive domain. And over the negative domain, $C_m(\cdot)$ is either nonnegative, or strictly increasing. \footnote{Detailed examples are provided in \cite{ xu2015demand}}.
    \end{itemize}
 \end{assumption}
We provide the following Lemma for the market clearing price and allocations as a function of SFE  $ \wbf^*$.
\begin{lemma} \label{lemma:SFE_C2}
 With Assumption \ref{assume:SFE_C1} \& \ref{assump:SFE_C2}, at a SFE $\wbf^*$:
\begin{itemize}
    \item the market clearing price is
    \beq
    \pi(\wbf^*)=B^{-1}(\frac{\mathbf{1}^\intercal \wbf^*}{\mathbf{1}^\intercal \Rbf-{\cal D}})
    \eeq
    which is a function of the bid-in parameter sum. 
    \item allocations of wholesale market participants are 
\beq
s_m(\pi(\wbf^*),w^*_m)=R_m- \frac{(\mathbf{1}^\intercal \Rbf - {\cal D})w^*_m }{\mathbf{1}^\intercal \wbf^*}, \forall m,\eeq
which is independent of $B(\cdot)$, and ${\cal D}$ is the inelastic demand in the wholesale market.
\end{itemize}
 \end{lemma}
% {\em Proof:} See Appendix. \hfill $\Box$
% This is a desirable scaling property for market mechanisms to be deployed in large-scale networks (Shenker 1990).
% \begin{lemma} \label{lemma:SFE_C1}
%  With $s_m(\pi,w_m)=R_m-\frac{w_m}{B(\pi)}, \forall m$, allocations of wholesale market participants at SFE $\wbf^*$ are 
% \beq
% s_m(\pi(\wbf^*),w^*_m)=R_m- \frac{(\mathbf{1}^\intercal \Rbf - {\cal D})w_m }{\mathbf{1}^\intercal \wbf}, \forall m,\eeq
% which is independent of $B(\cdot)$, and ${\cal D}$ is the inelastic demand in the wholesale market.
%  \end{lemma}
%  {\em Proof:} See Appendix. \hfill $\Box$
%  To make $\pi(\wbf)=0$ continuous, we have
%  \begin{assumption} \label{assump:SFE_Sdifferentiable}
% Assume $\pi(\wbf)=0$, $S=0$, when $\sum_{j=1}^M w_j= 0$. 
%  \end{assumption}
% Proof: $P_n=\frac{w_n}{B(\pi)}=\frac{w_n}{B(B^{-1}(\frac{\sum_n w_n}{D}))}= \frac{Dw_n }{\sum_j w_j}$. 
%So the market clearing allocations are proportional to the bids $w_n, \forall n$. 
See appendix for the proof. 

Denote $\Rbf_{-m}:=(R_1,...,R_{m-1},R_{m+1},...,R_M)$, $ {\cal J}_m(P_m):=1+\frac{{\cal M}P_m}{(1-{\cal M})P_m-D+R_{-m}}$. Assume the set $\{\wbf\succeq \mathbf{0}|s_m(\pi(\wbf),w_m)\in[\underline{P}_m, \bar{P}_m], \forall m\}$ is nonempty, we have the following theorem gives a efficient way to compute SFE and the optimal bidding parameter of a price maker DERA.
\begin{theorem}[{SFE and optimal price maker DERA bids}] \label{thm:SFE_C1}  With assumption \ref{assume:SFE_C1} \& \ref{assump:SFE_C2} and $|M| \geq 3$, the SFE for the wholesale market solves the optimal solution to the following  strictly convex optimization problem:
\begin{equation} \label{eq:SFE_thmC}
\begin{array}{lrl}&(P^*_m)_{m=1}^M=\underset{\mathbf{P}}{\rm arg ~min} & \sum_{m=1}^M \hat{C}_m(P_m)\\ 
& s.t. &\forall m\in\{1,...,M\}\\
&\pi^w:& \sum_{m=1}^MP_m={\cal D} ,\\
&&\underline{P}_m \le P_m\le \bar{P}_m.
\end{array}\end{equation}
% \beq
% \hat{C}_m(P_m)=C_m(P_m){\cal J}_m(P_m)-\int_0^{P_m}\frac{d {\cal J}_m(P_m)}{d P_m}C_n(y)dy,
% \eeq

When $P_m\geq 0$, $\hat{C}_m(P_m)=C_m(P_m){\cal J}_m(P_m)-\int_0^{P_m}\frac{d {\cal J}_m(P_m)}{d P_m}C_n(y)dy$; and when $P_m<0$, $\hat{C}_m(P_m)=C_m(P_m){\cal J}_m(P_m)+\int_{P_m}^0\frac{d {\cal J}_m(P_m)}{d P_m}C_n(y)dy$. And one optimal bidding parameter for price maker $m$ is  $w_m^*=B(\pi^*)(R_m- P_m^*)$.
% \beq
% \begin{array}{lrl}\label{eq:C_hat}
% \hat{C}_m(P_m)=\left\{\begin{matrix}C_m(P_m){\cal J}_m(P_m)-\int_0^{P_m}\frac{d {\cal J}_m(P_m)}{d P_m}C_n(y)dy,& if P_m\geq 0\\ C_m(P_m){\cal J}_m(P_m)+\int_{P_m}^0\frac{d {\cal J}_m(P_m)}{d P_m}C_n(y)dy,& if P_m<0\end{matrix}\right.,
% \end{array}\eeq

\end{theorem}
% {\em Proof:} See Appendix. \hfill $\Box$
% \textcolor{red}{add additional conditions for feasibility and existence. clarify conditions for prosumer utiltiy and DERA aggregation cost.}
See appendix for the proof. Note that to bound the integration in the formulation of $\hat{C}_m(P_m)$, we assume $|P_m| \le |\frac{{\cal D} -\sum_{j=1}^M R_j}{M-1}|, \forall m$ when ${\cal M}< 1$. Meanwhile, $|s_m(\pi(\wbf),w_m)|\le |\frac{{\cal D} -\sum_{j=1}^M R_j}{M-1}|, \forall m$ bounds $\wbf$. This will influence affine supply function with quadratic utility/cost \footnote{For linear supply function with ${\cal M}=-1$, $P_m\le ({\cal D} -\sum_{j=1}^M R_j)/2, \forall m$ is assumed for a bounded $\hat{C}_m(P_m)$ \cite{li2015demand}.}, but won't influence cases for log utility and isoelastic utility function. It's also shown in \cite{ndrio2022coordinated} that price makers will converge to the SFE through repeated bidding and market clearing procedures.

%  Note that for affine supply function $S_m(\pi, w_m)=R_m+w_m\pi$, assumption $P_m\le ({\cal D} -\sum_{j=1}^M R_j)/2, \forall m$ should be added for Theorem \ref{thm:SFE_C1} \cite{li2015demand}. 



